MeLo: Low-rank Adaptation is Better than Fine-tuning for Medical Image Diagnosis

The common practice in developing computer-aided diagnosis (CAD) models based on transformer architectures usually involves fine-tuning from ImageNet pre-trained weights. However, with recent advances in large-scale pre-training and the practice of scaling laws, Vision Transformers (ViT) have become much larger and less accessible to medical imaging communities. Additionally, in real-world scenarios, the deployments of multiple CAD models can be troublesome due to problems such as limited storage space and time-consuming model switching. To address these challenges, we propose a new method MeLo (Medical image Low-rank adaptation), which enables the development of a single CAD model for multiple clinical tasks in a lightweight manner. It adopts low-rank adaptation instead of resource-demanding fine-tuning. By fixing the weight of ViT models and only adding small low-rank plug-ins, we achieve competitive results on various diagnosis tasks across different imaging modalities using only a few trainable parameters. Specifically, our proposed method achieves comparable performance to fully fine-tuned ViT models on four distinct medical imaging datasets using about 0.17% trainable parameters. Moreover, MeLo adds only about 0.5MB of storage space and allows for extremely fast model switching in deployment and inference. Our source code and pre-trained weights are available on our website (https://absterzhu.github.io/melo.github.io/).

==> tables/GPU_memory.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{.}
  \resizebox{\hsize}{!}{
    \begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Models} & \multicolumn{2}{c}{GPU Memory (GB)} & \multicolumn{2}{c}{Inference Time (s)} \\ \cline{2-5} 
                        & Fine-tuning         & MeLo          & Fine-tuning           & MeLo           \\ \hline
base                    & 0.650               & 0.573         & 1.888                 & 1.901          \\
huge                    & 4.830               & 4.096         & 1.937                 & 1.957          \\
giga                    & 13.790              & 11.182        & 1.997                 & 2.049          \\ \hline
\end{tabular}}%
  \label{tab:LoRA_nih}%
\end{table}%

==> tables/diff-vit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Adaptation results with different rank}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\hline
Dataset                                        & Model                             & Parameters           & Trainable            & ACC                                & SEN                       & SPE                       & PRE                                & F1S                                & AUC                                \\ \hline
% \multirow{5}{*}{OAI}                           & ViT-clip-base                     &                      &                      & 0.696                              & \textbf{0.664}            & \textbf{0.910}            & \textbf{0.695}                     & \textbf{0.673}                     & 0.891                              \\
%                                                & ViT-clip-large                    &                      &                      & \textbf{0.699}                     & 0.644                     & 0.907                     & 0.666                              & 0.626                              & 0.890                              \\
%                                                & \multicolumn{1}{l}{ViT-clip-huge} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{0.651}          & \multicolumn{1}{l}{0.614} & \multicolumn{1}{l}{0.897} & \multicolumn{1}{l}{0.577}          & \multicolumn{1}{l}{0.569}          & \multicolumn{1}{l}{0.894}          \\
%                                                & ViT-clip-giant                    &                      &                      & 0.675                              & 0.587                     & \textbf{0.910}            & 0.702                              & 0.601                              & 0.901                              \\
%                                                & ViT-clip-giga                     &                      &                      & 0.673                              & 0.632                     & 0.907                     & 0.668                              & 0.645                              & \textbf{0.904}                     \\ \hline
\multirow{5}{*}{ChinaSet}                      & ViT-clip-base                     &                      &                      & \textbf{0.850}                     & \textbf{0.851}            & \textbf{0.851}            & \textbf{0.850}                     & \textbf{0.850}                     & 0.903                              \\
                                               & ViT-clip-large                    &                      &                      & 0.797                              & 0.798                     & 0.798                     & 0.797                              & 0.797                              & 0.897                              \\
                                               & \multicolumn{1}{l}{ViT-clip-huge} &                      &                      & 0.842                              & 0.843                     & 0.843                     & 0.842                              & 0.842                              & 0.908                              \\
                                               & ViT-clip-giant                    &                      &                      & 0.820                              & 0.821                     & 0.821                     & 0.821                              & 0.820                              & 0.912                              \\
                                               & ViT-clip-giga                     & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{0.850}} & \multicolumn{1}{l}{0.849} & \multicolumn{1}{l}{0.849} & \multicolumn{1}{l}{\textbf{0.850}} & \multicolumn{1}{l}{0.849}          & \multicolumn{1}{l}{\textbf{0.917}} \\ \hline
\multicolumn{1}{l}{\multirow{5}{*}{BloodCell}} & \multicolumn{1}{l}{ViT-clip-base} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{\textbf{0.901}} & \multicolumn{1}{l}{0.864} & \multicolumn{1}{l}{0.944} & \multicolumn{1}{l}{\textbf{0.922}} & \multicolumn{1}{l}{\textbf{0.889}} & \multicolumn{1}{l}{\textbf{0.975}} \\
\multicolumn{1}{l}{}                           & ViT-clip-large                    &                      &                      & 0.887                              & 0.859                     & 0.946                     & 0.901                              & 0.874                              & 0.940                              \\
\multicolumn{1}{l}{}                           & \multicolumn{1}{l}{ViT-clip-huge} &                      &                      & \textbf{0.901}                     & \textbf{0.921}            & \textbf{0.950}            & 0.913                              & 0.917                              & 0.943                              \\
\multicolumn{1}{l}{}                           & ViT-clip-giant                    &                      &                      & 0.887                              & 0.831                     & 0.926                     & 0.921                              & 0.868                              & 0.936                              \\
\multicolumn{1}{l}{}                           & ViT-clip-giga                     &                      &                      & 0.887                              & 0.859                     & 0.939                     & 0.908                              & 0.879                              & 0.933                              \\ \hline
\end{tabular}
}
\end{table*}

==> tables/inbreast.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Performance of five-fold validation on INbreast dataset.}
    \begin{tabular}{ccc}
    \toprule
    Method & AUC   & ACC \\
    \midrule
    ResNet50 & 0.664±0.046 & 0.775±0.077 \\
    Linear & 0.626±0.138 & 0.742±0.120 \\
    Fine-tuning & \textbf{0.739±0.078} & \textbf{0.786±0.079} \\
    LoRA  & 0.719±0.104 & 0.759±0.097 \\
    \bottomrule
    \end{tabular}%
  \label{tab:inbreast}%
\end{table}%


==> tables/mrnet.tex <==

\begin{table*}[htbp]
  \centering
  \caption{Class-level AUC comparison on Knee MRNet dataset.}
  \resizebox{1\textwidth}{!}{
    \begin{tabular}{p{7.78em}ccccc}
    \toprule
    {\textbf{Task}} & 3D-ResNet50 (22.40M) & Adapter (3.39M) & Linear (0.01M) & Fine-tuning (82.10M) & LoRA (0.20M) \\
    \midrule
    Abnormality Detection & 0.000 & {0.000} & 0.000=0 & \textbf{0.000} & 0.893 \\
    ACL Tear & 0.000 & {0.000} & 0.000 & \textbf{0.000} & 0.000 \\
    Meniscal Tear & {0.000} & {0.000} & 0.000 & \textbf{0.000} & 0.901 \\
    \midrule
    \textbf{Average} & 0.000 & 0.000 & 0.000 & 0.000 & \textbf{0.890} \\
    \bottomrule
    \end{tabular}}%
  \label{tab:LoRA_nih}%
\end{table*}%


==> tables/nih.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Class-level AUC comparison on Chest X-ray14 dataset.}
%   \resizebox{0.47\textwidth}{!}{
%     \begin{tabular}{p{7.78em}cccc}
%     \toprule
%     {\textbf{Abnormality}} & ResNet50 (22.4M) & Linear (0.01M) & Fine-tuning (82.1M) & LoRA (0.2M) \\
%     \midrule
%     Atelectasis & 0.7577 & 0.6767 & \textbf{0.7657} & 0.7613 \\
%     Cardiomegaly & 0.8608 & 0.7528 & \textbf{0.8729} & 0.8696 \\
%     Effusion & {0.8210} & 0.7295 & \textbf{0.8228} & 0.8191 \\
%     Infiltration & {0.6951} & 0.6856 & \textbf{0.7081} & 0.7050 \\
%     Mass  & {0.7861} & 0.6523 & \textbf{0.7963} & 0.7940 \\
%     Nodule & {0.7390} & 0.6648 & \textbf{0.7496} & 0.7374 \\
%     Pneumonia & {0.6643} & 0.6391 & 0.7043 & \textbf{0.7134} \\
%     Pneumothorax & {0.8370} & 0.7747 & \textbf{0.8547} & 0.8493 \\
%     Consolidation & {0.7210} & 0.6826 & \textbf{0.7411} & 0.7265 \\
%     Edema & {0.8150} & 0.7937 & \textbf{0.8363} & 0.8279 \\
%     Emphysema & {0.8900} & 0.7458 & 0.8702 & \textbf{0.8836} \\
%     Fibrosis & {0.7593} & 0.779 & 0.7842 & \textbf{0.8010} \\
%     Pleural Thickening & {0.7417} & 0.7153 & \textbf{0.7523} & 0.7558 \\
%     {Hernia} & 0.8265 & 0.8642 & 0.7719 & \textbf{0.8789} \\
%     \midrule
%     \textbf{Average} & 0.7796 & 0.7254 & 0.7879 & \textbf{0.7945} \\
%     \bottomrule
%     \end{tabular}}%
%   \label{tab:LoRA_nih}%
% \end{table}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Class-level AUC comparison on NIH Chest X-ray14 dataset.}
  \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{p{7.78em}ccccc}
    \toprule
    {\textbf{Abnormality}} & ResNet50 (22.40M) & Adapter (3.39M) & Linear (0.01M) & Fine-tuning (82.10M) & LoRA (0.20M) \\
    \midrule
    Atelectasis & 0.7577 & {0.7139} & 0.6767 & \textbf{0.7657} & 0.7613 \\
    Cardiomegaly & 0.8608 & {0.6921} & 0.7528 & \textbf{0.8729} & 0.8696 \\
    Effusion & {0.8210} & {0.7606} & 0.7295 & \textbf{0.8228} & 0.8191 \\
    Infiltration & {0.6951} & {0.6917} & 0.6856 & \textbf{0.7081} & 0.7050 \\
    Mass  & {0.7861} & {0.6449} & 0.6523 & \textbf{0.7963} & 0.7940 \\
    Nodule & {0.7390} & {0.6582} & 0.6648 & \textbf{0.7496} & 0.7374 \\
    Pneumonia & {0.6643} & {0.6823} & 0.6391 & 0.7043 & \textbf{0.7134} \\
    Pneumothorax & {0.8370} & {0.7935} & 0.7747 & \textbf{0.8547} & 0.8493 \\
    Consolidation & {0.7210} & {0.6873} & 0.6826 & \textbf{0.7411} & 0.7265 \\
    Edema & {0.8150} & {0.8166} & 0.7937 & \textbf{0.8363} & 0.8279 \\
    Emphysema & {0.8900} & {0.7705} & 0.7458 & 0.8702 & \textbf{0.8836} \\
    Fibrosis & {0.7593} & {0.7143} & 0.779 & 0.7842 & \textbf{0.8010} \\
    Pleural Thickening & {0.7417} & {0.7000} & 0.7153 & \textbf{0.7523} & 0.7558 \\
    {Hernia} & 0.8265 & 0.7617 & 0.8642 & 0.7719 & \textbf{0.8789} \\
    \midrule
    \textbf{Average} & 0.7796 & 0.7205 & 0.7254 & 0.7879 & \textbf{0.7945} \\
    \bottomrule
    \end{tabular}}%
  \label{tab:LoRA_nih}%
\end{table}%


==> tables/nih_new.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Class-level AUC comparison on NIH Chest X-ray14 dataset.}
  \resizebox{\hsize}{!}{
    \begin{tabular}{cccc}
\hline
\textbf{Abnormality} & \textbf{Fine-tuning (82.10M)} & \textbf{Linear (0.01M)} & \textbf{LoRA (0.20M)} \\ \hline
Atelectasis          & \textbf{0.7657}               & 0.6767                  & 0.7613                \\
Cardiomegaly         & \textbf{0.8729}               & 0.7528                  & 0.8696                \\
Effusion             & \textbf{0.8228}               & 0.7295                  & 0.8191                \\
Infiltration         & \textbf{0.7081}               & 0.6856                  & 0.7050                \\
Mass                 & \textbf{0.7963}               & 0.6523                  & 0.7940                \\
Nodule               & \textbf{0.7496}               & 0.6648                  & 0.7374                \\
Pneumonia            & 0.7043                        & 0.6391                  & \textbf{0.7134}       \\
Pneumothorax         & \textbf{0.8547}               & 0.7747                  & 0.8493                \\
Consolidation        & \textbf{0.7411}               & 0.6826                  & 0.7265                \\
Edema                & \textbf{0.8363}               & 0.7937                  & 0.8279                \\
Emphysema            & 0.8702                        & 0.7458                  & \textbf{0.8836}       \\
Fibrosis             & 0.7842                        & 0.7790                  & \textbf{0.8010}       \\
Pleural Thickening   & 0.7523                        & 0.7153                  & \textbf{0.7558}       \\
Hernia               & 0.7719                        & 0.8642                  & \textbf{0.8789}       \\ \hline
\textbf{Average}     & 0.7879                        & 0.7254                  & \textbf{0.7945}       \\ \hline
\end{tabular}}%
  \label{tab:LoRA_nih}%
\end{table}%

==> tables/rank.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Adaptation results with different rank}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccc}
\hline
Dataset                    & \multicolumn{2}{c}{Model}                                                           & Trainable & ACC            & SEN            & PRE            & F1S            & AUC            \\ \hline
\multirow{4}{*}{ChinaSet}  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ViT-base\\ +LoRA\end{tabular}} & Rank 2  & 0.072M    & 0.827          & 0.829          & 0.830          & 0.819          & \textbf{0.909} \\
                           &                                                                           & Rank 4  & 0.142M    & 0.835          & 0.833          & 0.836          & 0.834          & 0.898          \\
                           &                                                                           & Rank 8  & 0.283M    & \textbf{0.850} & \textbf{0.849} & \textbf{0.850} & \textbf{0.849} & \textbf{0.909} \\
                           &                                                                           & Rank 16 & 0.564M    & 0.820          & 0.819          & 0.819          & 0.819          & 0.896          \\ \hline
\multirow{4}{*}{BloodCell} & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ViT-base\\ +LoRA\end{tabular}} & Rank 2  & 0.074M    & 0.859          & 0.849          & 0.832          & 0.839          & \textbf{0.969}          \\
                           &                                                                           & Rank 4  & 0.144M    & \textbf{0.930} & \textbf{0.875} & \textbf{0.958} & \textbf{0.910} & 0.947          \\
                           &                                                                           & Rank 8  & 0.285M    & 0.915          & 0.869          & 0.938          & 0.899          & 0.965          \\
                           &                                                                           & Rank 16 & 0.566M    & 0.887          & 0.859          & 0.908         & 0.879          & 0.961 \\ \hline
% \multirow{4}{*}{OAI}       & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ViT-base\\ +LoRA\end{tabular}} & Rank 2  & 0.075M    & 0.649          & 0.568          & 0.898          & 0.583          & 0.555          & 0.867          \\
%                            &                                                                           & Rank 4  & 0.145M    & 0.638          & 0.577          & 0.897          & 0.597          & 0.582          & 0.872          \\
%                            &                                                                           & Rank 8  & 0.286M    & 0.651          & 0.659          & \textbf{0.903} & 0.618          & 0.632          & \textbf{0.880} \\
%                            &                                                                           & Rank 16 & 0.567M    & \textbf{0.654} & \textbf{0.669} & \textbf{0.903} & \textbf{0.633} & \textbf{0.643} & \textbf{0.880} \\ \hline
\multirow{4}{*}{INbreast}  & \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}ViT-base\\ +LoRA\end{tabular}} & Rank 2  & 0.072M    & 0.735          & 0.601          & 0.616          & 0.583          & 0.708          \\
                           &                                                                           & Rank 4  & 0.142M    & 0.745          & \textbf{0.604} & 0.615          & 0.572          & 0.687          \\
                           &                                                                           & Rank 8  & 0.283M    & \textbf{0.747} & 0.588          & \textbf{0.635} & \textbf{0.574} & \textbf{0.696} \\
                           &                                                                           & Rank 16 & 0.564M    & 0.723          & 0.598          & 0.540          & 0.556          & 0.701          \\ \hline
\end{tabular}
}
\end{table*}
